Geo-Indistinguishability: Differential Privacy for Location-Based Systems

The growing popularity of location-based systems, allowing unknown/untrusted servers to easily collect huge amounts of information regarding users' location, has recently started raising serious privacy concerns. In this paper we study geo-indistinguishability, a formal notion of privacy for location-based systems that protects the user's exact location, while allowing approximate information - typically needed to obtain a certain desired service - to be released. Our privacy definition formalizes the intuitive notion of protecting the user's location within a radius r with a level of privacy that depends on r, and corresponds to a generalized version of the well-known concept of differential privacy. Furthermore, we present a perturbation technique for achieving geo-indistinguishability by adding controlled random noise to the user's location. We demonstrate the applicability of our technique on a LBS application. Finally, we compare our mechanism with other ones in the literature. It turns our that our mechanism offers the best privacy guarantees, for the same utility, among all those which do not depend on the prior.

==> 6_census.tex <==
\section{Sanitizing datasets: US census case study}
\label{sec:census}

%\emph{private benefit versus social benefit}

%\emph{hiding confidence and hiding area -- masking confidence and masking area}

%emph{gelocation stand for geographic location (i.e. latitude and longitude coordinates}

%\emph{Make a point about the distinction between releasing a sanitized query answers vs releasing a sanitized dataset.}

In this section we present a sanitation algorithm for datasets containing geographical information. 
%Our algorithm achieves privacy guarantees by means of \emph{data perturbation techniques} which consist on adding random noise to the sensible geographic data. 
%
%Roughly speaking, the algorithm iteratively sanitizes each of the geographic sensitive values in the dataset by means of the perturbation technique presented in Section \ref{sec:mechanism}.% producing, in this way, a sanitized version of the dataset.
%
%% (we describe the algorithm in detail below). Another important feature of such algorithm is that allows us to easily trade privacy by utility (by modifying its privacy parameters). To the best of our knowledge, our algorithm constitutes the first privacy-aware sanitation approach for location-related datasets. 
%
%\subsection{The LODES dataset}
%
%%We illustrate the applicability of our algorithm by 
We consider a realistic case study involving publicly available data developed by the U.S Census Bureau's Longitudinal Employer-Household Dynamics Program  (LEHD).  These data, called LEHD Origin-Destination Employment Statistics (LODES), are used by {OnTheMap}, a web-based interactive %mapping 
application developed by the US Census Bureau. 
%The application enables, among other features, visualization of geographical information involving the residence and working location of US residents.
%(e.g., distance from home to work location). 

The LODES dataset includes information of the form $(hBlock , \allowbreak wBlock)$, where each pair represents a worker, the attribute $hBlock$ is the census block in which the worker lives, and $wBlock$ is the census block where the worker works. From this dataset it is possible to derive, by mapping home and work census blocks into their corresponding geographic centroids, a dataset with geographic information of the form ($hCoord$ , \allowbreak$wCoord$), where each of the coordinate pairs corresponds to a census block pair.

%Due to privacy constraints and legal issues, data involving the residence location of individuals cannot be released without previous sanitation; thus, the LODES dataset is a sanitized version of the real data. However, for illustration purposes and wlog, in the remaining of this section we will treat the LODES dataset as if it were the real data. 
The Census Bureau uses a \emph{synthetic data generation algorithm}  %\cite{Rubin:93:JOS}
\cite{Rubin:93:JOS, Machanavajjhala:08:ICDE}  
to sanitize the LODES dataset. Roughly speaking, the algorithm interprets the dataset as an histogram where each $(hBlock ,\allowbreak wBlock)$ pair is represented by a histogram bucket, the synthetic data generation algorithm sanitizes data by modifying the counts of the histogram. 
%For that purpose, a statistical model is built from the LODES dataset and then a sanitized counterpart is obtained by sampling points from the model. 
%(the details of the algorithm are described in [])

In the following we present a sanitizing algorithm for datasets with
geographical information (eg, the LODES dataset) that provides  geo-indistinguishability guarantees 
under the assumption that the home census blocks values in the
dataset are uncorrelated. Although this assumption weakens the
privacy guarantees provided by geo-indistinguishability, we believe that due to
the anonymizing techniques applied by the Census Bureau to the released data
involving census participants' information and to the large number of ($hCoord$,
$work\_coord$) pairs within small areas contained in the dataset, a practical
attack based on correlation of points is unlikely.

%In contrast to the sanitation algorithm used by the Census Bureau, 
%which modifies the counts of the LODES dataset seen as histogram, 
%our algorithm modifies the geographic data itself (in this case, following the approach of \cite{Machanavajjhala:08:ICDE}, the geographic data corresponding to residence locations -- in order to comply with the privacy constraints associated to such sensitive geographic data). 
%To the best of our knowledge, our algorithm defines the first sanitation mechanism for geographic information that provides formal privacy guarantees.


%\comment{Add references to the LODES data}

%Due to privacy constraints and legal issues, data involving workers' residential address cannot be released without . Instead, an anonymized version of the data is released. Therefore, the LODES data corresponds to the anonymized version of the original data.


%In the following we will show how to use our algorithm to pro

%
%

%For the remaining of this section we plan to first describe an anonymization algorithm that takes as an input a table of the form ($hCoord$,$work\_coord$) and outputs a table where the $hCoord$ points are anonymized one by one obtaining as a result formal guarantees for the resulting anonymized table. Then we will describe the formal guarantees provided by our algorithm and present experimental evidence of the utility of the resulting data. Finally, we will compare our approach with the approach used by the census bureau to annonymized the LODES original data.


%\subsection{The Sanitizing Algorithm for a dataset of locations}


%The algorithm takes as input (1) a dataset $D$ to sanitize, (2) the privacy parameters $\ell$  and $r$  (see Section \ref{sec:definitions}), and (3) the precision parameters $u$, $v$, $\delta_r$ and $\delta_\theta$, and the region $\cal A$. 
%(see Section \ref{sec:discrete}). The output of the algorithm is the sanitized counterpart of $D$. The algorithm is guaranteed to provide $\nicefrac{\ell}{r}$-geo-indistinguishability to the home coordinates of all individuals in the dataset (see discussion on protecting multiple locations in Section \ref{sec:multiple-locations}).
%The algorithm first determines $\epsilon=\nicefrac{\ell}{r}$.  Then for each $(c_h,c_w)\in D$, we
%generate a sanitized home coordinate $c_h'$ by using the $\mathit{NoisyPt}$ algorithm defined in Figure~\ref{fig:algo_point}.

Our sanitizing algorithm, described in Figure~\ref{fig:algo}, takes as input (1) a dataset $D$ to sanitize, (2) the privacy parameters $\ell$  and $r$  (see Section \ref{sec:definitions}), and (3) the precision parameters $u$, $v$, $\delta_r$ and $\delta_\theta$, and the region $\cal A$. 
(see Section \ref{sec:discrete}) and returns a sanitized counterpart of $D$. The algorithm is guaranteed to provide $\nicefrac{\ell}{r}$-geo-indistinguishability to the home coordinates of all individuals in the dataset (see discussion on protecting multiple locations in Section \ref{sec:multiple-locations}). 

%the level of protection $\epsilon'$ needed in order to guarantee $\epsilon=\nicefrac{\ell}{r}$ protection (see Theorem \ref{theo:geo-dp}), and the acceptable region $\cal A$ (see Section \ref{sec:truncation}). 
%We assume that  $\cal A$ contains all the home locations in $D$ and has a diameter not larger than 
%$r_{\max}  = \nicefrac{u}{\delta_\theta}$. Then for each $(c_h,c_w)\in D$, a radius $\rho$ and an angle $\theta$ are drawn 
%following the method in Figure~\ref{fig:method for the noise}.
%from the polar laplacian distribution  with parameter $\epsilon$ defined in \eqref{eqn:planar laplacian polar}. 
%The noise $(\rho,\theta)$ is then used to generate a sanitized home coordinate $c_h'$ on the reference system
%(see Section~\ref{sec:discrete}).
%%that is $r$ apart and at angle $\theta$ from the real home coordinate $c_h$. 
%Next, a test verification is performed in order to guarantee that  $c_h'$ lies in  $\cal A$ and, in case it does not, $c_h'$ is remapped to the closest point in $\cal A$ (see Section~\ref{sec:truncation}). 

%(We assume that the acceptable region $\cal A$ contains all the home locations in $D$ and has a diameter not larger than $r_{\max}$.)
%Finally, the new sanitized pair ($c_h',c_w$) is added to the output dataset $D'$.

\begin{figure}[tb]
\vspace{-0.3cm}
\centering
%\begin{center}
{\small
\begin{tabular}{l}
\hline\vspace{-0.3cm}\\
\textbf{Sanitizing Algorithm for a Dataset of Locations}\\ 
\hline \vspace{-0.3cm}\\ 
%
\textbf{Input:} $D : hCoord \times wCoord$ \codeComment{dataset to sanitize}\\ 
\hspace{0.9cm} $\ell$, $r$, $u$, $v$, $\delta_r$, $\delta_\theta$, ${\cal A}$   \codeComment{same as in Figure \ref{fig:algo_point}}\\
%
\textbf{Output:} Sanitized version  $D'$ of input $D$ \vspace{0.1cm}\\
%
1. \ \ $D'= \emptyset$; \codeComment{initializing output dataset}\\
2. \ \ $\epsilon= \nicefrac{l}{r};$\\
3. \ \ \textbf{for each} $(c_h,c_w)\in D$ \textbf{do}\\
4. \ \ \ \ \ \  $c_h'= {\mathit{NoisyPt}}(c_h,\epsilon, u, v, \delta_\theta, \delta_r, {\cal A})$;\codeComment{sanitized point}\\
5. \ \ \ \ \ \  $D'=D'\cup\{(c_h',c_w)\}$; \codeComment{adding sanitized point}\\
6. \ \ \textbf{end-for}\\
7. \textbf{return} $D'$;\\
\hline
\end{tabular}
}
%\vspace{-3mm}
%\end{center}
\smallskip
\caption{Our sanitizing algorithm, based on data perturbation}
\label{fig:algo}
%\vspace{-12pt}
\end{figure}

We note that, in contrast to the approach used by the Census Bureau based on histogram's count perturbation, our algorithm modifies the geographical data itself (residence coordinates in this case).  Therefore, our algorithm works at a more refined level than the synthetic data generation algorithm used by the Census Bureau; a less refined dataset can be easily obtained however -- by just remapping each $(hCoord , wCoord)$ pair produced by our algorithm to its corresponding census block representation.

In Appendix~\ref{app:experiments} we evaluate, via some experiments, the accuracy of the sanitized dataset generated by our algorithm. 



==> figures/plot/Makefile <==
DOC=plot

all: force
ps: $(DOC).ps
pdf: $(DOC).pdf

force: delete pdf
delete:
	rm -f $(DOC).pdf $(DOC).dvi $(DOC).ps $(DOC).tex



$(DOC).tex: $(DOC).plt
	gnuplot $(DOC).plt

$(DOC).dvi: $(DOC).tex
	latex $(DOC).tex
	#bibtex $(DOC)
	#latex $(DOC).tex

$(DOC).ps: $(DOC).dvi
	dvips -Pcmz $(DOC).dvi -o $(DOC).ps

$(DOC).pdf: $(DOC).ps
	ps2pdf $(DOC).ps

#$(DOC).pdf: *.tex
#	pdflatex $(DOC).tex
	#bibtex $(DOC)
	#pdflatex $(DOC).tex

clean:
	rm -f *.aux \
			*.log \
			*.toc \
			*.blg \
			*.bbl \
			$(DOC).dvi \
			$(DOC).tex \
			$(DOC).pdf \
			$(DOC).eps \
			$(DOC)-inc.eps \
			$(DOC).ps

